Double Multi-Head Attention for Speaker Verification

Most state-of-the-art Deep Learning systems for speaker verification are based on speaker embedding extractors. These architectures are commonly composed of a feature extractor front-end together with a pooling layer to encode variable-length utterances into fixed-length speaker vectors. In this paper we present Double Multi-Head Attention pooling, which extends our previous approach based on Self Multi-Head Attention. An additional self attention layer is added to the pooling layer that summarizes the context vectors produced by Multi-Head Attention into a unique speaker representation. This method enhances the pooling mechanism by giving weights to the information captured for each head and it results in creating more discriminative speaker embeddings. We have evaluated our approach with the VoxCeleb2 dataset. Our results show 6.09% and 5.23% relative improvement in terms of EER compared to Self Attention pooling and Self Multi-Head Attention, respectively. According to the obtained results, Double Multi-Head Attention has shown to be an excellent approach to efficiently select the most relevant features captured by the CNN-based front-ends from the speech signal.

==> DoubleMHA ICASSP 2021/glossary.tex <==
\newacronym{dl}{DL}{Deep Learning}
\newacronym{dbn}{DBN}{Deep Belief Network}
\newacronym{dnn}{DNN}{Deep Neural Network}
\newacronym{rbm}{RBM}{Restricted Boltzmann Machine}
\newacronym{cnn}{CNN}{Convolutional Neural Network}
\newacronym{rnn}{RNN}{Recurrent Neural Network}
\newacronym{lstm}{LSTM}{Long Short-Term Memory}
\newacronym{dbm}{DBM}{Deep Boltzmann Machine}
\newacronym{cd}{CD}{Contrastive Divergence}
\newacronym{urbm}{URBM}{Universal RBM}
\newacronym{udbn}{UDBN}{Universal DBN}
\newacronym{relu}{ReLU}{Rectified Linear Unit}
\newacronym{vrelu}{VReLU}{Variable ReLU}
\newacronym{ubm}{UBM}{Universal Background Model}
\newacronym{gmm}{GMM}{Gaussian Mixture Model}
\newacronym{map}{MAP}{Maximum a Posteriori}
\newacronym{nist}{NIST}{National Institute of Standard and Technology}
\newacronym{sre}{SRE}{Speaker Recognition Evaluation}
\newacronym{nap}{NAP}{Nuisance Attribute Projection}
\newacronym{jfa}{JFA}{Joint Factor Analysis}
\newacronym{lid}{LID}{Language Identification}
\newacronym{lda}{LDA}{Linear Discriminant Analysis}
\newacronym{vad}{VAD}{Voice Activity Detection}
\newacronym{plda}{PLDA}{Probabilistic Linear Discriminant Analysis}
\newacronym{wccn}{WCCN}{Within-Class Covariance Normalization}
\newacronym{asr}{ASR}{Automatic Speech Recognition}
\newacronym{det}{DET}{Detection Error Tradeoff}
\newacronym{eer}{EER}{Equal Error Rate}
\newacronym{dcf}{DCF}{Detection Cost Function}
\newacronym{mindcf}{minDCF}{minimum DCF}
\newacronym{far}{FAR}{False Acceptance Rate}
\newacronym{frr}{FRR}{False Rejection Rate}
\newacronym{fbe}{FBE}{Filter Bank Energy}
\newacronym{ff}{FF}{Frequency Filtering}
\newacronym{hmm}{HMM}{Hidden Markov Model}
\newacronym{lpc}{LPC}{Linear Predictive Coefficient}
\newacronym{lpr}{LPR}{Log Posterior Ratio}
\newacronym{mfcc}{MFCC}{Mel-Frequency Cepstral Coefficient}
\newacronym{lfcc}{LFCC}{Linear Frequency Cepstral Coefficient}
\newacronym{nn}{NN}{Neural Network}
\newacronym{pca}{PCA}{Principal Component Analysis}
\newacronym{plp}{PLP}{Perceptual Linear Predictive}
\newacronym{sdc}{SDC}{Shifted Delta Cepstrum}
\newacronym{psd}{PSD}{Power Spectral Density}
\newacronym{rbf}{RBF}{Radial Basis Function}
\newacronym{dct}{DCT}{Discrete Cosine Transform}
\newacronym{snr}{SNR}{Signal-to-Noise Ratio}
\newacronym{svm}{SVM}{Support Vector Machine}
\newacronym{cmn}{CMN}{Cepstral Mean Normalization}
\newacronym{cmvn}{CMVN}{Cepstral Mean and Variance Normalization}
\newacronym{cdf}{CDF}{Cumulative Distribution Function}
\newacronym{pdf}{pdf}{probability density function}
\newacronym{em}{EM}{Expectation-Maximization}
\newacronym{sv}{SV}{Speaker Verification}
\newacronym{sr}{SR}{Speaker Recognition}
\newacronym{an}{AN}{Adversarial Network}
\newacronym{en}{EN}{Encoding Network}
\newacronym{dn}{DN}{Discriminative Network}
\newacronym{mlp}{MLP}{Multilayer Perceptron}
\newacronym{gru}{GRU}{Gated Recurrent Unit}
\newacronym{tdnn}{TDNN}{Time Delay Neural Network}
\newacronym{nmt}{NMT}{Neural Machine Translation}
\newacronym{fc}{FC}{Fully Connected}
\newacronym{mha}{MHA}{Multi-Head Attention}
\newacronym{ams}{AMS}{Additive Margin Softmax}
\newacronym{tddn}{TDNN}{Time Delay Neural Network}

